Algorithms for Convex Quadratic Programming

The main contribution of this thesis is the development of a new algorithm for solving convex quadratic programs. It consists in combining the method of multipliers with an infeasible active-set method. Our approach is iterative. In each step we calculate an augmented Lagrange function. Then we minimize this function using an infeasible active-set method that was already successfully applied to similar problems. After this we update the Lagrange multiplier for the equality constraints. Finally we try to solve convex quadratic program directly, again with the infeasible active-set method, starting from the optimal solution of the actual Lagrange function. Computational experience with our method indicates that typically only few (most of the time only one) outer iterations (multiplier-updates) and also only few (most of the time less than ten) inner iterations (minimization of the Lagrange function) are required to reach the optimal solution. The diploma thesis is organized as follows. We close this chapter with some nota- tion used throughout. In Chapter 2 we show the equivalence of different QP problem formulations and present some important so-called direct methods for solving equality-constrained QPs. We cover the most important aspects for practically successful interior point methods for linear and convex quadratic programming in Chapter 3. Chapter 4 deals with ingredients for practically efficient feasible active set methods. Finally Chapter 5 provides a close description of our Lagrangian infeasible active set method and further gives a convergence analysis of the subalgorithms involved.

==> Active_set_methods.tex <==
\chapter{Active Set Methods}\label{ASM}





% Dantzigs's development of the simplex method in the late 1940s marks the start
% of the modern era in optimization. This method made it possible for economists
% to formulate large models and analyze them in a systematic and efficient
% way. Dantzigs's discovery coincided with the development of the first
% electronic computers, and the simplex method became one of the earliest
% important applications of this new and revolutionary technology. From those
% days to the present, computer implementations of the simplex method have been
% continually improved and refined. They have benefited particularly from
% interactions with numerical analysis, a branch of mathematics that also came
% into its own with the appearance of electronic computers, and have now reached
% a high level of sophistication. Today, linear programming and the simplex
% method continue to hold sway as the most widely used of all optimization tools
.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Diplomarbeit"
%%% End: 


==> DP_Introduction.tex <==
\chapter{Introduction}

preliminaries



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Diplomarbeit"
%%% End: 

